Analysis of Failures and Risks in Deep Learning Model Converters: A Case Study in the ONNX Ecosystem

Software engineers develop, fine-tune, and deploy deep learning (DL) models using a variety of development frameworks and runtime environments. DL model converters move models between frameworks and to runtime environments. Conversion errors compromise model quality and disrupt deployment. However, the failure characteristics of DL model converters are unknown, adding risk when using DL interoperability technologies. This paper analyzes failures in DL model converters. We survey software engineers about DL interoperability tools, use cases, and pain points (N=92). Then, we characterize failures in model converters associated with the main interoperability tool, ONNX (N=200 issues in PyTorch and TensorFlow). Finally, we formulate and test two hypotheses about structural causes for the failures we studied. We find that the node conversion stage of a model converter accounts for ~75% of the defects and 33% of reported failure are related to semantically incorrect models. The cause of semantically incorrect models is elusive, but models with behaviour inconsistencies share operator sequences. Our results motivate future research on making DL interoperability software simpler to maintain, extend, and validate. Research into behavioural tolerances and architectural coverage metrics could be fruitful.

==> oldcontent.tex <==
\section{OLD CONTENT}

%DL Intermediate Formats:
\paragraph{DL Intermediate Formats}
%\textbf{DL Intermediate Formats:}
%Intermediate formats are a common intermediary to interoperate DL software.
Common DL intermediate formats are Open Neural Network eXchange (ONNX)~\citep{ONNXFixed}, NNEF~\citep{NNEF}, and MMdnn~\citep{MMdnn}.
ONNX has the broadest adoption (\cref{tab:intermediate_formats}). %, with 
%ONNX boasts the most stars, forks, dependants, and packages utilizing it.


\paragraph{Interoperability is for deployment} 
Model converters can serve multiple purposes.
They can convert from an intermediate representation back to a development framework (``upstream'' for further development).
They can also convert from a development framework to an intermediate representation (``downstream'' for deployment). 
This is analogous to how compiler techniques can be used for compilation and de-compilation.

To understand which engineering use cases predominate in DL interoperability, we examined Stack Overflow.
  1,148 StackOverflow posts included the keyword ``ONNX''.
We randomly sampled 10\% (120 posts) and categorized them based on the author's apparent goal.
Six analysts were trained on a pilot set of posts, then analyst pairs categorized 40 posts each. %the author's overall goals.
%Three raters The categorization process involved three pairs of raters, who had the 120 posts divided amongst them and assigned goals to the posts. 
% For a subset of posts (120), we categorize the goal of the author. We divide the 120 posts among 3 pairs of raters and categorize posts according to their goal.
Given that this was not the focus of our study, we only report the result where the raters agreed (see~\cref{sec:DataAvailability} for details).
As~\cref{tab:stackoverflow} shows, most questions --- and thus, we infer, common ONNX uses --- are for model deployment.

\begin{table}
\caption{
  \PJ{REPLACE WITH WENXIN SURVEY DATA} Goals of ONNX posts on StackOverflow. %belonging to the category Conceptual, Development, Deployment, Unclear, or N/A.
  }
\small
  \vspace{-0.25cm}
\begin{tabular}{cr}
\toprule
\textbf{Goal} 
& \textbf{\# Posts}  
\\ \hline
Conceptual  
& 1  
\\
Development
& 1  
\\
Deployment       
& 36
\\
Unclear
& 27
\\
N/A
& 2
\\
\midrule
\textbf{Total} 
& 67
\\
\bottomrule
\end{tabular}
\label{tab:stackoverflow}
\end{table}

\paragraph{ONNX} % \& converters
In DL software, the most prominent implementation of Wegner's common intermediary pattern is the Open Neural Network eXchange, ONNX.
% \footnote{Other common intermediaries are MMDnn~\citep{XXX} and NNEF~\citep{XXX} \url{https://www.khronos.org/nnef}. Neither has achieved widespread use.}
ONNX was introduced by Facebook and Microsoft in 2017.


% \begin{table}[]
% \caption{TABLE YOU WANTED}
% \begin{tabular}{lrrr}
% \toprule
% {} &  \code{tf2onnx} &  pytorch &  total \\
% \midrule
% API Misuse                      &        7 &       10 &     17 \\
% Incompatability                 &       38 &       49 &     87 \\
% Type Problem                    &       32 &       49 &     81 \\
% Shape Problem                   &       14 &       16 &     30 \\
% Incorrect Numerical Computation &        0 &        1 &      1 \\
% Incorrect Assignment            &        2 &        4 &      6 \\
% Incorrect Exception Handling    &        1 &        5 &      6 \\
% Misconfiguration                &        5 &        2 &      7 \\
% Concurrency                     &        0 &        0 &      0 \\
% Algorithmic Error               &       21 &       12 &     33 \\
% Typo                            &        1 &        2 &      3 \\
% Testing                         &        2 &       10 &     12 \\
% Documentation                   &        1 &        2 &      3 \\
% Others                          &       14 &       11 &     25 \\
% \bottomrule
% \end{tabular}
% \end{table}



\begin{table}[h]
%\begin{wraptable}{r}{0.70\columnwidth}
\caption{
\small
    Adapted taxonomy of failure symptoms~\citep{DLcompilerbugs}.
    \emph{Emphasis}: wording changed.
    \emph{Hang} symptom omitted (unobserved).
    \JD{Table formatting}
    \JD{Wenxin, the changes here are so simple that I don't think it's worth the space to include. Move it to the Appendix. In the paper itself, just list the symptoms inline in a paragraph labeled `Taxonomy of Symptoms'. The interesting ones are `wrong model' and `bad performance', so write a full sentence for each of those. The rest are self-explanatory.}
}
  % Reduce font size?
  \small
  \footnotesize
\begin{tabular}{cp{6cm}}
\toprule
\textbf{Symptom} & \textbf{Definition} \\
\toprule
Crash           & The \emph{model converter} terminates unexpectedly during \emph{conversion}, usually producing an error message. \\
Wrong \emph{Model}     & The \emph{model converter} behaves unexpectedly without crashing, producing a wrong intermediate or final result. \\
Bad Performance & The time cost or memory consumption of the \emph{model converter} is much larger than developer/user expectations (\eg the performance achieved on the previous version during regression testing or performance achieved by certain hardware). \\
Build Failure   & Installation of \emph{model converter} or dependencies fails. \\
Unreported      & The symptom cannot be identified by analyzing the corresponding issues including code changes, discussions, and related issues. \\
\iffalse
%JD: Below this is the Hang symptom that we did not observe
\midrule
\midrule
Hang            & This symptom means that the \emph{converter} keeps running for a long period of time without producing the expected result. \\
\fi
\bottomrule
\end{tabular}
\label{tab:taxonomy_symptoms}
%\vspace{-0.35cm}
\end{table}
%\end{wraptable}




\subsection{Results} \label{sec:theme2-results}

\subsubsection{Result for H1: Do Opsets affect failure modes?}\label{sec:result:H1}




\begin{center}
    ======== OLD CONTENT =========
\end{center}

\subsubsection{Method for H2: What model attributes result in failures?}\label{sec:meth:RQ3}

% To answer \textbf{RQ3}, we measure the current failure rate and symptoms (\cref{tab:symptoms}) of these ONNX converters.
To answer \textbf{H2}, we test DL converters with a variety of inputs and analyze the characteristics of failure-inducing inputs. 
\cref{fig:TwoPartMethodForRQ3} illustrates our two-stage process, which we detail next.

\iffalse
We convert two types of models to capture both typical and unusual input regimes:
  real-world DL models from Jiang \etals{} \code{HFTorrent} dataset~\citep{Jiang2022PTMReuse, jiang_empirical_2023, Jiang_Banna_Vivek_Goel_Synovic_Thiruvathukal_Davis_2023}
  and
  synthetic models generated systematically~\citep{NNSmith}. 
%These models represent the spectrum of possible input, both expected and improbable.
We convert each model with its respective converter.
The conversion may fail (\eg crash).
If the converted model loads in the ONNX Runtime, we use differential testing~\citep{mckeeman1998differential} to measure conversion quality. % between original and converted models.
%For failing models, we submit GitHub issues to the respective repositories.
We analyze the characteristics of failing models.
Specifically, we analyze the operator types and operator sequences --- we justify our choices in \cref{todo}. 
And their operator and operator sequences to identify shared features.
Additionally, we compare with models that do not fail and determine if operators or operator sequences are shared.
\fi

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.43\textwidth}
    \includegraphics[width=\columnwidth]{figures/illustrations/conversions.png}
    \caption{
      Inference behavior pre-/post-conversion.
    }
    \label{fig:MethodForRQ3DifferentialTest}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.50\textwidth}
    \includegraphics[width=\columnwidth]{figures/illustrations/RQ3_Method.png}
    \caption{
      Causal analysis of misbehavior.
    }
    \label{fig:MethodForRQ3CausalAnalysis}
  \end{subfigure}
  \caption{
      (a) \textbf{Conversion differential test}: Models are converted using \code{tf2onnx} or \code{torch.onnx} as appropriate.
      If conversion succeeds, differences are measured between original and converted model.
      (b) \textbf{Mismatching model analysis}: \circledstep{1} For two sets of models we compare all simple paths between two models. The common operator sequences are depicted in the intersection. 
      \circledstep{2} is found by comparing models with the set of mismatched models. 
      It contains all sequences that are shared by mismatching models. 
      \circledstep{3} is found by comparing models from the mismatched and correct model sets.
      It contains all sequences that are shared between correct and mismatched models.
      \circledstep{4} is found by comparing models from the mismatched and test suite sets. 
      It contains all sequences that are shared between correct and mismatched models.
  }
  \label{fig:TwoPartMethodForRQ3}
\end{figure}

\paragraph{Differential Test (\cref{fig:MethodForRQ3DifferentialTest})}

For a differential test, we need to select (1) inputs, and (2) a criterion for ``too different''~\citep{mckeeman_differential_1998}.

\textbf{Inputs:} For inputs, we converted both real models and synthetic models.
Real models contain input patterns that the converter expects. 
Synthetic models are more diverse and should exercise edge cases on the converter.
Our sources of real and synthetic models were:
% Real models are inputs that converters are likely to see.
% Synthetic models are inputs that converters would not see (fuzzing).
% Saying the converters would not see synthetic models may make the reviewer ask why they are important.
\begin{itemize}[leftmargin=10pt]
    \item \textit{Real Models:}
        We used the HFTorrent dataset from Jiang \etal~\citep{Jiang2022PTMReuse}.
        This is the largest available set of real-world DL models, containing \HFTorrentTotalRepos pre-trained models collected from the HuggingFace Model Zoo. 
        We filtered for the \TotalHFModels models with both PyTorch and TensorFlow versions, allowing comparison between the two converters on similar inputs.
        These models represent \HFDistinctArch distinct full architectures (\HFArchitectures backbones).
    \item \textit{Synthetic Models:}
        We systematically generated synthetic DNNs for conversion, using the \code{NNSmith} tool~\citep{NNSmith}.
        \code{NNSmith} generates random valid TensorFlow and PyTorch DNNs that use operators supported by ONNX.
        We added a parameter to \code{NNSmith} to generate DNNs of a given size (\# nodes).
        We then \textit{systematically generated DNNs containing between \GenLowerBound-\GenUpperBound nodes in increments of \GenIncrements}.
        For each node count, we generated DNNs until two conditions were met:
          (1) All \code{NNSmith}-supported operators appeared at least once in the family;
          and
          (2) $\geq$ \GenUpperBound distinct models were created.
\end{itemize}

    In initial tests, we found the resulting models were often convertible yet unsupported by ONNX~RunTime (\cref{tab:RQ4ConversionResults}).
    To address the common forms of ONNX Runtime errors for \code{torch.onnx}, we constrained the NNSmith synthesizer.
    % (\cref{tab:RQ4ConversionConstrainedResults}).
    Specifically, we removed \PTOpsRemoved operator out of \PTOps for \code{torch.onnx} and \TFOpsRemoved out of \TFOps for \code{tf2onnx}. 
    \PJ{Double check the totals}.
    Additionally, we confined the tensor data type to \code{float32}.

    There are other DL model generation approaches, \eg 
      MUFFIN~\citep{Muffin_Gu_Luo_Zhou_Wang_2022},
      COMET~\citep{COMET_Li_Cao_Tian_Tsz_On_Li_Wen*_Cheung*_2023},
      and
      LEMON~\citep{LEMON_Wang_Yan_Chen_Liu_Zhang_2020}.
    These tools generate inputs by mutating seed models, typically real models.
    We viewed HFTorrent as a sufficient source of real models, and synthesized with~\code{NNSmith} because it is more random.
    %We discuss its limitations in~\cref{sec:Threats}.

\textbf{Difference Criterion:}
For each model, we attempt to convert it to ONNX using its respective converter.\footnote{For the real models, we used the HuggingFace converter. This converter performs some preprocessing and then invokes \code{torch.onnx} or \code{tf2onnx}. For synthetic models, we invoked the respective converters directly.} % --- \code{torch.onnx} for PyTorch and \code{tf2onnx} for TensorFlow. 
If conversion succeeds, we load it into the ONNX~RunTime.
For models that load successfully, we perform inference on both the original model (using PyTorch or TensorFlow) and the converted model (using ONNX Runtime).
For \emph{real} models, we use the inputs provided by the model owners to test the model.
  These are called ``dummy inputs'' in HuggingFace packages.
For \emph{synthetic} models, we use 100 randomly generated inputs matching the model's input shape.

In both cases, to measure model misbehavior we used a simple and community-accepted approach:
  the distance measure and threshold used by the PyTorch exporter. % one distance measure to compare the output tensors from the original and converted models:
This rule is that \textit{between the original and ONNX-converted models, in the inference result tensors, the maximum absolute element-wise difference should be smaller than $10^{-7}$}
~\citep{pytorch_onnx_verification}.
% ~\citep{huggingface_export_validation}

We considered alternatives to measure behavioral differences.
% We acknowledge that there are many other ways to measure model behavioral differences.
A more general notion of tolerance or ``acceptable error'' could be used, but the choice of tolerance is not well established --- the PyTorch verification tool uses $10^{-7}$, NNSmith uses $10^{-3}$~\citep{NNSmith}.
% , and HuggingFace uses $10^{-7}$.
Openja \etal~\citep{ConvertingDLempirical} proposed using model accuracy and robustness,
\ifJOURNALEXTENSION
\footnote{Though related, there is a distinction between the predictions of the model and the accuracy of a model. The ``accuracy'' of a model is the performance of a model on a dataset, whereas the predictions are the outputs of the model. A model with accuracy differences (relative to an oracle) would necessarily mean that there are differences in the predictions, but the inverse is not necessarily true.}
\fi 
but this method requires training each model on a suitable dataset.
Training substantially increases the cost of the measurement, and the dataset requirement limits the types of models that can be generated.
% \JD{This is a fact, but we also need to give the rationale/reasons why it's hard to decide as well. Methods sections must answer both What and Why. Apply this principle throughout your methods sections, not just here.}
% \TODO{We received many comments about "accuracy loss" / "correct" behaviour in the last review. It would be worthwhile to quantify why this is the case }
  % and the L1 and L2 measures.
%We consider the converted and original models identical if the max absolute difference $< 10^{-3}$.
%This follows the thresholds used by HuggingFace~\citep{huggingface_transformers_serialization}.

\iffalse
% FIGURE 5
\begin{wrapfigure}{r}{0.61\columnwidth}
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/illustrations/conversions.png}
    \caption{
    Conversion test.
    Models are converted using \code{tf2onnx} or \code{torch.onnx} as appropriate.
    If conversion succeeds, differences are measured between original and converted model.
    }
    \label{fig:MethodForRQ4}
    %\vspace{-0.35cm}
\end{wrapfigure}
\fi

\PJ{METHOD FOR H3}
\paragraph{Model Causal Analysis} % (\cref{fig:MethodForRQ3CausalAnalysis})} \label{sec:meth:model_analysis}
Given the challenges in interpreting the behaviors of DNNs, particularly across two different representations, we instead evaluate two causal hypotheses: \emph{incorrect conversions result from (\textbf{H1}) operator types and (\textbf{H2}) operator sequences}. 
%Here we explain our method to evaluate them.
These hypotheses derive from our results in Theme 1, so we defer the rationale to~\cref{sec:res:RQ3}. % (specifically, Findings \TODO{X,Y,Z} in \cref{sec:Results}). 
%\emph{Node Type} and \emph{Algorithmic Errors} are common --- \eg \TODO{Some examples from Theme 1} --- indicating that both the types of operators and their sequences of them play a part in failures.

We test these hypotheses by analyzing DL models along the two pertinent dimensions, of operator types and operator sequences.
For operator type analysis we count all operator types present in mismatched, correct, and test suite models. 
% \JD{This paragraph only describes sequences, what about operator types? A simple table would be nice to include in the Results, showing whether or not we can point to a set of operators that commonly occur only in mismatching models.} 
For sequence analysis, see~\cref{fig:MethodForRQ3CausalAnalysis}.
% \cref{fig:MethodForRQ3CausalAnalysis} depicts our sequence analysis.
We compare pairs of models from two sets and extract all common sequences between the two sets of models \circledstep{1}.
For each model in a pair, we find all simple paths from the inputs to the outputs. 
The simple paths of the two models are compared and common sequences are extracted (a common sequence is a sequence of shared operators of length $>2$).\footnote{A simple path is a string. A common sequence is its substring. We process simple paths as strings in our implementation.}
We find the following common sequences: 
% between mismatched models \circledstep{2}, mismatched and correct models \circledstep{3}, and mismatched and test suite models \circledstep{4}.
\circledstep{2} all sequences that mismatched models share; 
\circledstep{3} all sequences that are shared by correct and mismatched models (by \textbf{H2}), these sequences are not the cause of mismatches);
\circledstep{4} all sequences that test suites share with the mismatching models.

The utilization of simple paths for analysis has inherent limitations. 
Simple paths provide sequences of operations from inputs to outputs and cannot capture conversions that are branching.
\cref{fig:graph_comp} depicts such a case. 
% The conversion of the \code{max} node results in the \code{ReduceMax} and \code{ArgMax} nodes. 
The simple paths of the ONNX model would produce two sequences containing the \code{ReduceMax} and \code{ArgMax} nodes, respectively, but this is confounding.
A node conversion that results in multiple nodes is not captured (semantically) under such analysis.
% \JD{Discuss limitation here of simple paths. Also refer back to Figure 2 for an example.}

The common sequences between two sets of models may be largely identical.
This can inflate the number of ``unique'' sequences there actually are. 
For example, the sequences \code{aaaabd} and \code{aaaabc} are identical except for the last element.
To deal with cases we further reduce the common sequences to the smallest shared subsequences, \ie we recursively find the longest common subsequences for our sequences until we cannot find any smaller subsequences~\citep{algo_cormen2022introduction}.
% The algorithm is given in~\cref{lst:reduced_sub_matching}.

\paragraph{Hypothesis Testing} \label{sec:meth:hypothesis_testing}
Given this data, we test the two hypotheses.
To evaluate \textbf{H1}, the impact of \emph{operator types}, we compare the operators of mismatched and correct models.
If mismatched model operators overlap with correct model operators ops, we \emph{reject} this hypothesis. 
To evaluate \textbf{H2}, the impact of \emph{operator sequences}, we identify all shared operator sequences belonging \emph{only} to mismatched models, and determine how common they are. 
% and test the most commonly shared sequence.
To resolve this hypothesis:
  (a) if sequences are not commonly shared by mismatched models, we reject the hypothesis;
  (b) if sequences are rarely shared among mismatched models, the result is inconclusive;
  and
  (c) if many mismatching models share the same sequences, this supports our hypothesis.
% If the sequences are not common to the majority of models
% we reject the hypothesis.~\PJ{Explain.}
% , and if the sequences, individually, or under composition are not erring,
% We build models and test conversions as follows: (1) 10 models made of a single common sequence, and (2) 10 simple paths containing the most commonly found sequence.
% , \circledstep{2} $-$ (\circledstep{2} $-$ \circledstep{3}) --- reducing the sequences as described in~\cref{sec:meth:model_analysis}. 

% \begin{wrapfigure}{r}{0.5\textwidth}
% \centering
% \begin{minipage}{\textwidth}
% \small
% \begin{lstlisting}[style=algorithmstyle, caption={Recursive Substring Matching Pseudo-Python. The implementation makes use of the SequenceMatcher class from the Python Standard Library.}, label={lst:reduced_sub_matching}]
% # Inputs: seqs: a list of sequences; seq_len: length of seqs
% # Output: A list of sequences containing the smallest.
% def recursive_submatching(seqs, seq_len):
%     submatches = set(seqs)
%     for seq_a, seq_b in combinations(seqs): # choose 2 combinations
%         matching_subseqs = all_matching_subseqs(seq_a, seq_b)
%         for subseq in matching_subseqs:
%             if subseq.size > 3:
%                 submatches.add(match_1)
%                 if seq_a in submatches:
%                     submatches.remove(i)
%                 if seq_b in submatches:
%                     submatches.remove(j)
%     if seq_len - submatches.length > 0:
%         return recursive_submatching(submatches, submatches.length)
%     return seqs
% \end{lstlisting}
% \end{minipage}
% \end{wrapfigure}

% FIGURE 6 
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.75\columnwidth]{figures/illustrations/RQ3 Method.png}
%     \caption{
%     Model Analysis. 
%     \circledstep{1} For two sets of models we compare all simple paths between two models. The common operator sequences are depicted in the intersection. 
%     \circledstep{2} is found by comparing models with the set of mismatched models. 
%     It contains all sequences that are shared by mismatching models. 
%     \circledstep{3} is found by comparing models from the mismatched and correct model sets.
%     It contains all sequences that are shared between correct and mismatched models.
%     \circledstep{4} is found by comparing models from the mismatched and test suite sets. 
%     It contains all sequences that are shared between correct and mismatched models.
%     }
%     \label{fig:MethodForRQ3Analysis}
%     %\vspace{-0.35cm}
% \end{figure}


\iffalse
\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\columnwidth]{figures/illustrations/conversions.png}
    \caption{
      \textbf{Conversion test.}
      Models are converted using \code{tf2onnx} or \code{torch.onnx} as appropriate.
      If conversion succeeds, differences are measured between original and converted model.
      % \PJ{@Arav can you try to subfig this next to Fig 6.}
      % \JD{Nit: Write Real (HFTorrent) and Synthetic (NNSmith)}
      % \AT{I can't get this to work someone help plz :(}
    }
    \label{fig:MethodForRQ4}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\columnwidth]{figures/illustrations/RQ3_Method.png}
    \caption{
      \textbf{Model Analysis.} 
      \circledstep{1} For two sets of models we compare all simple paths between two models. The common operator sequences are depicted in the intersection. 
      \circledstep{2} is found by comparing models with the set of mismatched models. 
      It contains all sequences that are shared by mismatching models. 
      \circledstep{3} is found by comparing models from the mismatched and correct model sets.
      It contains all sequences that are shared between correct and mismatched models.
      \circledstep{4} is found by comparing models from the mismatched and test suite sets. 
      It contains all sequences that are shared between correct and mismatched models.
    }
    \label{fig:MethodForRQ3Analysis}
  \end{subfigure}
  \caption{Conversion test and model analysis.}
\end{figure}
\fi

\subsubsection{Method for RQ4: Characteristics of test suites}
\label{sec:meth:testSuites}
To analyze converter test suites, we examined continuous integration/deployment (CI/CD) pipelines.
We noted testing practices and collected any models used for testing. 
These models are analyzed as one of the groups of models considered in~\cref{fig:MethodForRQ3CausalAnalysis}.
Since this task was reasonably objective, the analysis was performed by one researcher.


% \subsection{Results} \label{sec:theme2-results}

\subsection{RQ3: Characteristics of Failing Models} \label{sec:res:RQ3}

%%%%%%%%%%%
% \begin{table*}[ht!]
%     \caption{
%     Results of conversion testing.
%     For real models, conversion may fail in the HuggingFace wrapper.
%     Both kinds of models may fail in the DL model converter, or when the result is loaded into the ONNX Runtime (ORT).
%     %\emph{Crash (converter)} is a crash during model conversion.
%     %\emph{Crash (ORT)} is a crash in the loading of a \emph{successfully} converted model into ONNX Runtime.
%     \emph{Incorrect Outputs} are when any ORT inference result exceeds the allowed distance of $10^{-3}$. 
%     Real models rarely fail.
%     Synthetic models often fail.
%     }
%    % Reduce font size?
%    %\small
%     \begin{tabular}{l|rrr|rrr}
%     \toprule
%     \multirow{2}{*}{\textbf{Outcome}}   &  \multicolumn{3}{c}{\emph{\textbf{\code{tf2onnx}}}} &  \multicolumn{3}{c}{\emph{\textbf{\code{torch.onnx}}}} \\
%                     &         \textbf{Real} & \textbf{Syn.} &  \textbf{Syn. Con.} &      \textbf{Real}   & \textbf{Syn.} & \textbf{Syn. Con.} \\
%     \midrule
%     \emph{Start: Number of models} &        \TotalHFModels &   \TotalRandModelTF &  \TotalTFConGen &  \TotalHFModels & \TotalRandModelPT & \TotalPTConGen\\
%     % Successful      &        \SuccessHFTF &   \SuccessNNTF &    \SuccessHFPT & \SuccessNNPT\\
%     Unsuccessful Conversion (HF error) &    \CrashesHFTFHugging & N/A & N/A & \CrashesHFPTHugging & N/A & N/A \\
%     \midrule
%     Unsuccessful Conversion        &          \CrashesHFTF &      \CrashesNNTF & \ConvCrashTFConGen &     \CrashesHFPT &  \CrashesNNPT & \ConvCrashPTConGen \\
%     Unsuccessful ORT loading  & \CrashesORTHFTF & \CrashesORTNNTF & \ORTCrashTFConGen& \CrashesORTHFPT &  \CrashesORTNNPT & \ORTCrashPTConGen \\ 
%     Incorrect Output     &       \FailureHFTFSemantic &     \FailureNNTFSemantic &  \SemanticTFConGen &     \FailureHFPTSemantic &     \FailureNNPTSemantic & \SemanticPTConGen\\
%     % \midrule
%     % \midrule
%     Successful      &        \TrueSuccessHFTFM &   \TrueSuccessNNTF & \SuccessfulTFConGen &    \TrueSuccessHFPTM & \TrueSuccessNNPT & \SuccessfulPTConGen\\
    
%     % Unique Crashes &   \UnqCrashesHFTF & 0 & \UnqCrashesHFPT & \UnqCrashesNNPT\\
%     % \midrule\midrule
%     % Diff. Tested &  - & \DiffTestedNNTF & \DiffTestedHFPT & \DiffTestedNNPT\\    
%     % \midrule\midrule
%     \bottomrule
%     \end{tabular}
%     \label{tab:RQ4ConversionResults}
% %\vspace{-0.15cm}
% \end{table*}

% Smaller Table
%%%%%%%%%%%
% \begin{table*}[ht!]
%     \caption{
%     Results of conversion testing.
%     For real models, conversion may fail in the HuggingFace wrapper.
%     Both kinds of models may fail in the DL model converter, or when the result is loaded into the ONNX Runtime (ORT).
%     %\emph{Crash (converter)} is a crash during model conversion.
%     %\emph{Crash (ORT)} is a crash in the loading of a \emph{successfully} converted model into ONNX Runtime.
%     \emph{Incorrect Outputs} are when any ORT inference result exceeds the allowed distance of $10^{-3}$. 
%     Real models rarely fail.
%     Synthetic models often fail.
%     }
%    % Reduce font size?
%    %\small
%     \begin{tabular}{l|r|r}
%     \toprule
%     {\textbf{Outcome}}   &  {\emph{\textbf{\code{tf2onnx}}}} & {\emph{\textbf{\code{torch.onnx}}}} \\
%                     % &        \textbf{Syn. Con.} &      \textbf{Syn. Con.} \\
%     \midrule
%     \emph{Start: Number of models} &   \TotalTFConGen & \TotalPTConGen\\
%     % Successful      &        \SuccessHFTF &   \SuccessNNTF &    \SuccessHFPT & \SuccessNNPT\\
%     Unsuccessful Conversion   &    \ConvCrashTFConGen &   \ConvCrashPTConGen \\
%     Unsuccessful ORT loading  & \ORTCrashTFConGen &  \ORTCrashPTConGen \\ 
%     Incorrect Output     &     \SemanticTFConGen &   \SemanticPTConGen\\
%     % \midrule
%     % \midrule
%     Successful      &   \SuccessfulTFConGen & \SuccessfulPTConGen\\
    
%     % Unique Crashes &   \UnqCrashesHFTF & 0 & \UnqCrashesHFPT & \UnqCrashesNNPT\\
%     % \midrule\midrule
%     % Diff. Tested &  - & \DiffTestedNNTF & \DiffTestedHFPT & \DiffTestedNNPT\\    
%     % \midrule\midrule
%     \bottomrule
%     \end{tabular}
%     \label{tab:RQ4ConversionResults}
% %\vspace{-0.15cm}
% \end{table*}

\iffalse
\begin{table*}[hb]
\centering
    \begin{minipage}{0.49\textwidth}
    \centering
    \caption{
    TESTING. Results of conversion testing.
    For real models, conversion may fail in the HuggingFace wrapper.
    Both kinds of models may fail in the DL model converter, or when the result is loaded into the ONNX Runtime (ORT).
    %\emph{Crash (converter)} is a crash during model conversion.
    %\emph{Crash (ORT)} is a crash in the loading of a \emph{successfully} converted model into ONNX Runtime.
    \emph{Incorrect Outputs} are when any ORT inference result exceeds the allowed distance of $10^{-3}$. 
    Real models rarely fail.
    Synthetic models often fail.
    }
   % Reduce font size?
   \small
    \begin{tabular}{l|rr|rr}
    \toprule
    \multirow{2}{*}{\textbf{Outcome}}   &  \multicolumn{2}{c}{\emph{\textbf{\code{tf2onnx}}}} &  \multicolumn{2}{c}{\emph{\textbf{\code{torch.onnx}}}} \\
                    &         \textbf{Real} &  \textbf{Syn.} &      \textbf{Real}  & \textbf{Syn.} \\
    \midrule
    \emph{Start: Number of models} &        \TotalHFModels &  \TotalTFConGen &  \TotalHFModels & \TotalPTConGen\\
    % Successful      &        \SuccessHFTF &   \SuccessNNTF &    \SuccessHFPT & \SuccessNNPT\\
    Unsuccessful Conversion (HF error) &    \CrashesHFTFHugging & N/A & \CrashesHFPTHugging & N/A \\
    \midrule
    Unsuccessful Conversion        &          \CrashesHFTF & \ConvCrashTFConGen &     \CrashesHFPT & \ConvCrashPTConGen \\
    Unsuccessful ORT loading  & \CrashesORTHFTF & \ORTCrashTFConGen & \CrashesORTHFPT & \ORTCrashPTConGen \\ 
    Incorrect Output     &       \FailureHFTFSemantic &  \SemanticTFConGen &     \FailureHFPTSemantic & \SemanticPTConGen\\
    % \midrule
    % \midrule
    Successful      &        \TrueSuccessHFTFM & \SuccessfulTFConGen &    \TrueSuccessHFPTM & \SuccessfulPTConGen\\
    
    % Unique Crashes &   \UnqCrashesHFTF & 0 & \UnqCrashesHFPT & \UnqCrashesNNPT\\
    % \midrule\midrule
    % Diff. Tested &  - & \DiffTestedNNTF & \DiffTestedHFPT & \DiffTestedNNPT\\    
    % \midrule\midrule
    \bottomrule
    \end{tabular}
    \label{tab:RQ4ConversionResults}
%\vspace{-0.15cm}
    \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
    \centering
    \caption{
    TESTING
    Results of conversion testing.
    For real models, conversion may fail in the HuggingFace wrapper.
    Both kinds of models may fail in the DL model converter, or when the result is loaded into the ONNX Runtime (ORT).
    %\emph{Crash (converter)} is a crash during model conversion.
    %\emph{Crash (ORT)} is a crash in the loading of a \emph{successfully} converted model into ONNX Runtime.
    \emph{Incorrect Outputs} are when any ORT inference result exceeds the allowed distance of $10^{-3}$. 
    Real models rarely fail.
    Synthetic models often fail.
    }
   % Reduce font size?
   \small
    \begin{tabular}{l|rr|rr}
    \toprule
    \multirow{2}{*}{\textbf{Outcome}}   &  \multicolumn{2}{c}{\emph{\textbf{\code{tf2onnx}}}} &  \multicolumn{2}{c}{\emph{\textbf{\code{torch.onnx}}}} \\
                    &         \textbf{Real} &  \textbf{Syn.} &      \textbf{Real}  & \textbf{Syn.} \\
    \midrule
    \emph{Start: Number of models} &        \TotalHFModels &  \TotalTFConGen &  \TotalHFModels & \TotalPTConGen\\
    % Successful      &        \SuccessHFTF &   \SuccessNNTF &    \SuccessHFPT & \SuccessNNPT\\
    Unsuccessful Conversion (HF error) &    \CrashesHFTFHugging & N/A & \CrashesHFPTHugging & N/A \\
    \midrule
    Unsuccessful Conversion        &          \CrashesHFTF & \ConvCrashTFConGen &     \CrashesHFPT & \ConvCrashPTConGen \\
    Unsuccessful ORT loading  & \CrashesORTHFTF & \ORTCrashTFConGen & \CrashesORTHFPT & \ORTCrashPTConGen \\ 
    Incorrect Output     &       \FailureHFTFSemantic &  \SemanticTFConGen &     \FailureHFPTSemantic & \SemanticPTConGen\\
    % \midrule
    % \midrule
    Successful      &        \TrueSuccessHFTFM & \SuccessfulTFConGen &    \TrueSuccessHFPTM & \SuccessfulPTConGen\\
    
    % Unique Crashes &   \UnqCrashesHFTF & 0 & \UnqCrashesHFPT & \UnqCrashesNNPT\\
    % \midrule\midrule
    % Diff. Tested &  - & \DiffTestedNNTF & \DiffTestedHFPT & \DiffTestedNNPT\\    
    % \midrule\midrule
    \bottomrule
    \end{tabular}
    \label{tab:RQ4ConversionResults}
    \end{minipage}
%\vspace{-0.15cm}
\end{table*}
\fi

%%%%%%%%%%%%%
\begin{table*}[hb]
    \caption{
    Results of conversion testing.
    Real models' conversion may fail in the HuggingFace wrapper.
    Both kinds of models may fail in DL model converter, or when the result is fed to ONNX Runtime (ORT).
    %\emph{Crash (converter)} is a crash during model conversion.
    %\emph{Crash (ORT)} is a crash in the loading of a \emph{successfully} converted model into ONNX Runtime.
    \emph{Behavioural Difference}: ORT inference results with difference $> 10^{-7}$. 
    Real models fail rarely, synthetic models often.
    % \JD{Needs percentages}
    }
    \vspace{-5pt}
   % Reduce font size?
   \small
    \begin{tabular}{l|rr|rr}
    \toprule
    \multirow{2}{*}{\textbf{Outcome}}   &  \multicolumn{2}{c}{\emph{\textbf{\code{tf2onnx}}}} &  \multicolumn{2}{c}{\emph{\textbf{\code{torch.onnx}}}} \\
                    &         \textbf{Real} &  \textbf{Syn.} &      \textbf{Real}  & \textbf{Syn.} \\
    \midrule
    \emph{Start: Number of models} &        \TotalHFModels &  \TotalTFConGen &  \TotalHFModels & \TotalPTConGen\\
    % Successful      &        \SuccessHFTF &   \SuccessNNTF &    \SuccessHFPT & \SuccessNNPT\\
    Unsuccessful Conversion (HF error) &    \CrashesHFTFHugging (\CrashesHFTFHuggingPercent) & N/A & \CrashesHFPTHugging (\CrashesHFPTHuggingPercent) & N/A \\
    \midrule
    Unsuccessful Conversion        &          \CrashesHFTF (\CrashesHFTFPercent) & \ConvCrashTFConGen (\ConvCrashTFConGenPercent) &     \CrashesHFPT (\CrashesHFPTPercent) & \ConvCrashPTConGen (\ConvCrashPTConGenPercent) \\
    Unsuccessful ORT loading  & \CrashesORTHFTF (\CrashesORTHFTFPercent) & \ORTCrashTFConGen (\ORTCrashTFConGenPercent) & \CrashesORTHFPT (\CrashesORTHFPTPercent) & \ORTCrashPTConGen (\ORTCrashPTConGenPercent) \\ 
    Behavioural Difference     &       \FailureHFTFSemantic (\FailureHFTFSemanticPercent)  &  \SemanticTFConGen (\SemanticTFConGenPercent) &     \FailureHFPTSemantic (\FailureHFPTSemanticPercent) & \SemanticPTConGen (\SemanticPTConGenPercent)\\
    % \midrule
    % \midrule
    Successful      &        \TrueSuccessHFTFM (\TrueSuccessHFTFMPercent) & \SuccessfulTFConGen (\SuccessfulTFConGenPercent) &    \TrueSuccessHFPTM (\TrueSuccessHFPTMPercent) & \SuccessfulPTConGen (\SuccessfulPTConGenPercent)\\
    
    % Unique Crashes &   \UnqCrashesHFTF & 0 & \UnqCrashesHFPT & \UnqCrashesNNPT\\
    % \midrule\midrule
    % Diff. Tested &  - & \DiffTestedNNTF & \DiffTestedHFPT & \DiffTestedNNPT\\    
    % \midrule\midrule
    \bottomrule
    \end{tabular}
    \label{tab:RQ4ConversionResults_BIG}
%\vspace{-0.15cm}
\end{table*}
%%%%%%%%%%%%%

%%%
\begin{tcolorbox} [width=\linewidth, colback=yellow!30!white, top=1pt, bottom=1pt, left=2pt, right=2pt]
\textbf{Finding 7}: 
Real models convert well: converter crashes and incorrect behavior affected only $\sim$5\% of models.

% \textbf{Finding 8}: 
% Constraining the synthetic model generation substantially reduced the generation of models with expected incompatibilities, from 2,985 to 1,017.

\textbf{Finding 8}: 
Synthetic models reveal incorrect model behavior more often than Real models, with  \FailureSemanticTotalSyn/\TotalSynModel ($\sim$\IncorrectTotalSynPercentage\%) of synthetic models exhibiting this compared to \FailureHFSemanticTotal/\TotalRealModels real models ($\sim$\IncorrectTotalRealPercentage\%).

\textbf{Finding 9}:
  \textbf{\textit{H1}} failed: Incorrect conversions are not (simply) due to the use of unusual operators.
  \textbf{\textit{H2}} was inconclusive: we did not observe strong correlation between the use of unusual operator sequences and conversion failures.
\end{tcolorbox}

% Recap what we did.
From our results in Theme 1, we hypothesize that incorrect conversions are the results of both (\textbf{H1}) operator types, as well as (\textbf{H2}) the sequence of operators in a model. 
We are motivated by the fact that \emph{Node Type} and \emph{Algorithmic Errors} are common causes of error. 
Both causes pertain to how nodes or node sequences are handled during conversion. 
Thus diverse node types and node sequences should induce errors, and specifically, certain node types and sequences would be more likely to cause errors, \ie we expect to see failing models share characteristics.
We test these hypotheses as discussed in \cref{sec:Methods-Theme2}. 
We convert both real and synthetic models using the \code{tf2onnx} and \code{torch.onnx} model converters.
% We test the \code{tf2onnx} and \code{torch.onnx} model converters using both real and synthetic models.
% Recall that we generated synthetic models in two ways: constrained only for the frameworks (default NNSmith) and with additional constraints for limitations of the ONNX Runtime.
\cref{tab:RQ4ConversionResults} contain our testing results following the outline given in~\cref{fig:MethodForRQ3DifferentialTest}.
\cref{tab:RQ4AnalysisResultsNodes} and \cref{tab:RQ4AnalysisResultsSeq} contain the results of our node and sequence analysis, respectively.
  % for default NNSmith, 
  %and
  %\cref{tab:RQ4ConversionConstrainedResults} shows the results with additional constraints.

% \JD{Structure should match what I put in place in 4.3.1: subsubsection called ``Results of Differential Test'', and subsubsection called ``Results of Causal Hypothesis''. Use paragraphs below that.}


\subsubsection{Results for Differential Test (H2)}
\paragraph{Results for Real Models}

Real models exhibited few converter failures and little incorrect model behavior.
Most issues occurred within the HuggingFace-specific converter.
Converter failures occurred for only \ConverterFailures/\ConverterAttempted models ($\sim$\ConverterFailuresPercentage\%).
Once models reached \code{torch.onnx} and \code{tf2onnx}, over \ConverterSuccessPercentage\% could be converted and exhibited equivalent behavior in the ONNX Runtime.

We note that the dataset of real models we used included many that shared an architecture and differed only in weights (\ie checkpoints of the same model).
We were surprised to observe that the different weights alone were enough to produce different behaviors in our evaluation.
For example, in \code{tf2onnx}, various checkpoints of the \code{t5} model
  had 65 HuggingFace conversion errors,
  56 unsuccessful \code{tf2onnx} conversions,
  1 unsuccessful ONNX Runtime load,
  0 incorrect outputs,
  and
  183 successes.
We could not find an explanation for this instability. It bears further investigation.

% The model authors
% %know of the inconsistent behavior in ONNX and
% attribute this to ``implementation differences''~\citep{sharma2021primera}.

\paragraph{Results for Synthetic Models}

As described in~\cref{sec:Methods-Theme2}, we systematically generated models using our adaptation of the NNSmith tool.
% , with and without constraining for the ONNX Runtime.
Results varied substantially from real models. 
% \JD{unclear --- of what? / from what? ``between real and synthetic models''?}.

% \paragraph{Difficulties in Converting and Loading:}

Synthetic models exhibit difficulties when converting to ONNX and when loading the converted model to the ONNX Runtime.
We find that \emph{Unsuccessful Conversions} occur \TotalConvCrash times, almost entirely in synthetic models on \code{tf2onnx}.
The \TotalConvCrash crashes correspond to \UnsucessfulUniqueCrashes unique crashes.
% , both of which involve \emph{``no complex type support''}~\citep{pytorchissue59246}.
Of the \SuccessConvNN synthetic models that successfully convert, only \SuccessLoadNN successfully load into ONNX Runtime. 

% \JD{Anonymization issues here. Please Slack me if you are unsure how to write this.}
In this experiment, we independently identified both known and novel defects.
% \JD{This paragraph talks about ORT errors but not conversion errors, I'm not sure if it is exhaustive or not?}
We observed \ORTUnique unique ONNX Runtime errors, of which 6 appear to correspond to open GitHub issues~\citep{pytorchissue78721, ONNX Runtime9760, ONNX Runtime17061, ONNX Runtime11846, ONNX Runtime12302, ONNX Runtime12594}.
%returned with \ORTTypeMismatch.
We disclosed the rest to the engineering teams.
% ~\citep{tf2onnx2235, tf2onnx2247, pytorch109806, ONNX Runtime17616}. 
For most disclosures, we have not yet received a response. 
For one disclosure, which described a model that causes the \code{libc++ abi} to terminate unexpectedly during inference with ONNX Runtime, the response was that it had been (unintentionally) fixed in the development branch.
It still affects older releases. 
% One is similar to type mismatch errors in~\citep{pytorchissue78721}.
% We could not identify open GitHub issues corresponding to the others.

% We found that these difficulties were mitigated by constraining the model generation process to account for ONNX Runtime issues.
% These constraints reduced instances of
%   \emph{Unsuccessful ORT loading}
%   from \CrashesORTNNTF to \ORTCrashTFConGen for \code{tf2onnx} and from \CrashesORTNNPT to \ORTCrashPTConGen for \code{torch.onnx}. 
% This indicates that constraining model generators enables end-to-end testing of DL model converters (cf. ~\cref{sec:dis:conv_test}).
% We developed the constraints based on ONNX Runtime failures after the \code{torch.onnx} converter; these were apparently inadequate for the \code{tf2onnx} and bear further study.

% We find that convsec:dis:conv_test crash $\sim$9\% \WJ{Do we have exact numbers here? I don't think $\sim$ is a good way to present our data.}of the time (\cref{tab:RQ4ConversionResults}).
% This is a shift downward from what we measure in \cref{sec:rov:rq}
% Of this 9\% \code{torch.onnx} contributes $\sim$66\% of crashes whereas \code{tf2onnx} contributes the remaining $\sim$33\%.
% We find that the \code{torch.onnx} converter crashes at approximately equal amounts for synthetic and real inputs --- \CrashesHFPT and \CrashesNNPT, respectively.
% This does not play out for \code{tf2onnx} which exclusively crashes for \code{real} inputs, with all models successfully converting for the \code{tf2onnx} converter.

% Upon closer examination, we find that many of these crashes throw the same exception at the same line number and same file. 
% Controlling for this we find that in total there were only \TotalUniqueCrashes unique crashes.  
% Of the \TotalUniqueCrashes we find that three of these errors the crashes being known \emph{Incompatibilities} in the PyTorch converter:\WJ{Should this be a comma? Three types: a, b, and c? Maybe I misunderstood.} \textit{no complex type support}~\citep{pytorchissue59246} and \textit{aten::scatter\_reduce}~\citep{pytorchissue84260}.
% \href{https://github.com/pytorch/pytorch/issues/59246}{no complex type support} and \href{https://github.com/pytorch/pytorch/issues/84260}{aten::scatter\_reduce} \TODO{Convert to citations}.
% The remaining unique crashes are a result of the original model

% \paragraph{Behavioral Differences:}
We observed a large fraction of behavioural differences (incorrect output) with synthetic models. % with constrained synthetic models revealing the most for the \code{torch.onnx} converter.
Compared to real models, which had \FailureHFSemanticTotal instances, synthetic models had \FailureSemanticTotalSyn instances where the inference results exceeded the threshold from~\cref{sec:meth:RQ3}.
% Almost all of these instances were observed only for the constrained synthetic models.
The majority of these instances were observed in the \code{tf2onnx} converter.
For both converters, we disclosed such instances to the respective engineering teams (we have not heard a response yet). %~\footnote{Blinded for submission.} 

\ifJOURNALEXTENSION
\begin{table}[h]
  \centering
  \small
  \caption{
  Table describing the issue.
  }
  \begin{tabular}{c|c|c|c|}
    \toprule
    \textbf{Description} & \textbf{Symptom} & \textbf{Location} & \textbf{Conjectured cause} \\
    \hline
    \code{tf2onnx} segfaults during conversion & Crash & ... & protobuf size limit \\
    \code{tf2onnx} segfaults during conversion & Crash & ... & protobuf size limit \\
    
    \bottomrule
  \end{tabular}
  \label{tab:mytable}
\end{table}
\fi

%(\FailureSemanticTotalSynPT/\FailureSemanticTotalSyn) with \SemanticPTConGen/\FailureSemanticTotalSynPT being found by constrained synthetic models.
%This leads us to conclude that synthetic models may provide benefits over real models~\cref{sec:dis:conv_test}.

\begin{table*}[ht!]
    \centering
% \begin{wraptable}{r}{0.45\columnwidth}
    \caption{
    Model Operator Analysis Results.
    As described in~\cref{sec:meth:model_analysis}: 
    Mismatched \circlestep{a}
, all operators that mismatched models contain; 
    Correct (b) all operators that correct models contain;
    Test Suite (c) all operators that test suites contain.
    (a) - (b) are all operators in (a) but not in (b).
    (b) - (a) are all operators in (b) but not in (a).
    (a) - (c) are all operators in (a) but not in (c).
    (c) - (a) are all operators in (c) but not in (a).
    % \circledstep{4} - \circledstep{2} are all unique sequences that are \emph{only} present in test suite models.
    % The reduced sequences are found by applying the reduction as described in~\cref{sec:meth:model_analysis}
    }
    \vspace{-5pt}
   % Reduce font size?
   \small
    \begin{tabular}{c|r|r}
    \toprule
    \textbf{Model Type}   &  \emph{\textbf{\code{tf2onnx}}} &  \emph{\textbf{\code{torch.onnx}}} \\
    \midrule
    Mismatched (a) &   54  & 58 \\
    Correct (b) &    52  & 59 \\
    Test Suite (c)&   54 & 16\\
    \midrule
    (a) - (b)&   0  & 1 \\
    (b) - (a)&   2  & 0 \\
    (a) - (c) &   21  & 46 \\
    (c) - (a) &   21  & 4 \\
    \bottomrule
    \end{tabular}
    \label{tab:RQ4AnalysisResultsNodesOld}
%\vspace{-0.15cm}
\end{table*}
% \end{wraptable}

\begin{table*}[b!]
    \centering
    \caption{
    Model Sequence Analysis Results.
    As described in~\cref{sec:meth:model_analysis}: 
    \circledstep{2} all sequences that mismatched models share; 
    \circledstep{3} all sequences that are shared by correct and mismatched models;
    \circledstep{4} all sequences that test suites share with the mismatching models.
    \circledstep{2} - \circledstep{3} are all unique sequences that are \emph{only} present in mismatched models.
    % \circledstep{4} - \circledstep{2} are all unique sequences that are \emph{only} present in test suite models.
    The reduced sequences are found by applying the reduction as described in~\cref{sec:meth:model_analysis}.
    }
    \vspace{-3pt}
   % Reduce font size?
   \small
    \begin{tabular}{c|rr|rr}
    \toprule
    \multirow{2}{*}{\textbf{Set}}   &  \multicolumn{2}{c}{\emph{\textbf{\code{tf2onnx}}}} &  \multicolumn{2}{c}{\emph{\textbf{\code{torch.onnx}}}} \\
                    &   \textbf{Unique Sequences} & \textbf{Reduced Sequences} &      \textbf{Unique Sequences} & \textbf{Reduced Sequences} \\
    \midrule
    \circledstep{2} &    2,125 & 1,126 & 980 & 635 \\
    \circledstep{3} &    1,050 & 508 & 4,243 & 2,988 \\
    \circledstep{4} &    35 &  35 & 2 & 2\\
    \midrule
    \circledstep{2} - \circledstep{3} &      1,527 & 862 & 176 & 131\\
    % \circledstep{2} - \circledstep{4} &       2,135 & 1,097 & 979 & 637\\
    \bottomrule
    \end{tabular}
    \label{tab:RQ4AnalysisResultsSeqOld}
%\vspace{-0.15cm}
\end{table*}


\subsubsection{Results of Causal Hypotheses (}
As described in~\cref{sec:meth:model_analysis} we analyze both the operator type and operator sequences for various sets of models, in particular, we examine synthetic models.
We compare three sets of models: correct models, mismatched models, and test suite models (discussed in~\cref{sec:res:RQ4}).

% \JD{State which hypothesis is being considered and what your conclusion is}
% We find that incorrect conversions do not result simply from operator types.
Our analysis reveals that incorrect conversions are not related simply to the types of nodes present.
\cref{tab:RQ4AnalysisResultsNodes} contains the results of our node analysis.
We collect and compare the operator types in the mismatched, correct, and test suite models.
We find, of the 154 ONNX operators, 
(1) mismatched models contain 58 (\code{torch.onnx}) and 54 (\code{tf2onnx}) unique operator types, whereas,
(2) correct models contain 59 (\code{torch.onnx}) and 52 (\code{tf2onnx}) unique operator types. 
% (3) test suite models contain 16 (\code{torch.onnx}) and 54 (\code{tf2onnx}) unique operator types.
There is a significant overlap between operators in correct and mismatched models.
Almost all operators are shared save for 1 (\code{torch.onnx}) and 2 (\code{tf2onnx}), indicating that for synthetic models operator types may not be determinant of mismatch.
% Test suite models on the other hand shared 12 operators (\code{torch.onnx}) and 33 (\code{tf2onnx}) with mismatched models.
% For \code{tf2onnx}: 
% (1) correct models contain 52 unique operator types; 
% (2) mismatched models contain 54 unique operator types;
% (3) test suite models contain 57 unique operator types.
% There is a significant overlap between operators in correct and mismatched models.
% Almost all operators are shared save for 1, indicating that at least for synthetic models node types may not be determinant of mismatch.
% Test suite models on the other hand only shared 35 operators with mismatched models.

Our analysis reveals that incorrect conversions cannot be attributed simply to node sequences --- our hypothesis is inconclusive.
% We find that incorrect conversions are not simply a result of the node sequences.
\cref{tab:RQ4AnalysisResultsSeq} contains the results of our sequence analysis.
We find that mismatched models, \circledstep{2}, share many operator sequences, 2,125 (\code{tf2onnx}) and 980 (\code{torch.onnx}).
Moreover, mismatched models and correct models, \circledstep{3}, also share many sequences --- 1,050 (\code{tf2onnx}) and 4,242 (\code{torch.onnx}).
% Test suite and mismatched models, \circledstep{4}, do not.
% The \code{tf2onnx} test suite only sharing 35 sequences with mismatched models, whereas the \code{torch.onnx} only sharing 2. 
% We discuss implications in~\cref{sec:dis:WhyOfFailure}.
When we compare how many sequences are present only in mismatched models, \circledstep{2} - \circledstep{3}, \code{tf2onnx} has 1,527 sequences, whereas \code{torch.onnx} has 176.
After reduction \code{tf2onnx} and \code{torch.onnx} contain 862 and 131 sequences, respectively.
Now, remember that, as described in~\cref{sec:meth:hypothesis_testing}, 
% if reduced sequences are not shared by the majority of mismatching models then we reject the hypothesis.
if sequences are not commonly shared by mismatched models, we reject the hypothesis; (b) if sequences are shared among some models, our hypothesis is inconclusive; and (c) if sequences are shared across the majority of models our hypothesis is supported.
We find that for \code{torch.onnx}, only 1 of the 131 sequences is shared by more than 3 models, and for \code{tf2onnx} no sequence is shared by more than 11 models.
This indicates there may be a family of sequences that can cause errors and thus our hypothesis is inconclusive.


\ifJOURNALEXTENSION
Constraining synthetic models is effective at revealing incorrect model behavior post-conversion, this is for the \code{torch.onnx} converter.
The effect of constraining models results in more models being able to be loaded into ORT, as seen in \cref{tab:RQ4ConversionResults}.
We find that 728 of the 7,192 synthetically generated models exhibit inference result differences, with the majority being by synthetic models that were constrained.
Constrained \code{torch.onnx} models more often revealed incorrect model behavior, with \SemanticPTConGen/\SuccLoadedPTConGen ($\sim$37\%) as compared to unconstrained which had \FailureNNPTSemantic/\SuccLoadedPTSyn ($\sim$24\%).
We do not measure this for \code{tf2onnx} where though more models successfully were loaded into ONNX Runtime this did not result in measuring more models which exhibited incorrect behavior.
\fi

% In comparing the inference results of converted models to their original counterparts.
% % We compare the inference results using ONNX Runtime (ORT) of the successfully converted models with their original models (given the same inputs).
% We find that \TotalDiffTestFail /\TotalAttempted (\WJ{percent?}) models had outputs greater than the threshold \WJ{What is the threshold? Let's mention it again here.} specified in \cref{sec:mod_conv_test}.
% This corresponds to a 
% \emph{Real} PyTorch models being different from their converted models \FailureHFPTSemantic /\TotalDiffTestFail times, with these failures corresponding to two architectures: Longformer Encoder-Decoder (LED) and Longformer --- the authors of the model attribute this to ``implementation differences''~\citep{sharma2021primera}.
% Comparatively, \emph{synthetic} models exhibit this more often \emph{real} models making up \FailureNNSemantic /\TotalDiffTestFail. 
% \WJ{Why synthetic models fail more in the inference? We should have some explanations here. Is this a pitfall on converters, ORT, or NNSmith?}

% \subsubsection{Comparison to Retrospective Failures (\cref{sec:res:RQ1})}
% Compared to our retrospective analysis, this prospective analysis provides a distinctly different view of the distribution failure symptoms. 
% Combining real and synthetic model results, we find that only \CrashTotalPercentage\% of tested models crashed at the converter (low likelihood), while \IncorrectTotalPercentage\% exhibited incorrect output (higher likelihood).
% In comparison, in our retrospective analysis, crashes make up $\sim$\CrashPercent of issues analyzed and incorrect behavior is $\sim$\WrongModelPercent(\cref{sec:res:RQ1}).
% Retrospective analysis captures the criticality of failures, but not their likelihood.
% When comparing the \emph{Wrong Model} symptoms that we found in \cref{sec:res:RQ1} to such instances in 

\ifJOURNALEXTENSION
% Present Data
\subsubsection{Issues with Model Loading in Compilers}\TODO{Merge with 5.4.3 and talk about constrained generation}
In attempting to do this we find that only \TotalAttempted of the \TotalSuccessForDiff that successfully converted were able to load into ORT --- mainly belonging to \emph{real} models.  
We discuss the implications of this with respect to converter testing in \cref{sec:dis:conv_test}.
\fi

\iffalse
\begin{table}[hbt!]
    \caption{
    \TODO{UPDATE THIS IS FOR CONSTRAINED GENERATION}
    Failures in Conversion Testing.
    \emph{Crash (converter)} crash during model conversion.
    \WJ{We should be consistent between this caption and subsection headings. 5.4.1 is crashes which should include the crash (ORT). Maybe think about change the headings to ``Converter Crash'' and ``Runtime Crash''?}
    \emph{Crash (ORT)} is a crash in the loading of a \emph{successfuly} converted model into ONNX Runtime.
    \emph{Incorrect Outputs} are when the inference results have a max absolute difference between original and converted models greater than  $<$ $10^{-3}$.
    We were unable to test \emph{real} tf2onnx models using ONNX Runtime.
    }
    \begin{tabular}{l|r|r}
    \toprule
    {Outcome}   & {\code{tf2onnx}} &  {\code{torch.onnx}} \\
    \midrule
    Generated           &        \TotalTFConGen &   \TotalPTConGen \\
    % Successful      &        \SuccessHFTF &   \SuccessNNTF &    \SuccessHFPT & \SuccessNNPT\\
    Unsuccessful Conversion   &   \ConvCrashTFConGen &    \ConvCrashPTConGen\\
    Crash (ORT)  & \ORTCrashTFConGen & \ORTCrashPTConGen \\ 
    Incorrect Output     &      \SemanticTFConGen &     \SemanticPTConGen  \\
    % \midrule
    % \midrule
    Successful      &        \SuccessfulTFConGen &   \SuccessfulPTConGen\\
    
    % Unique Crashes &   \UnqCrashesHFTF & 0 & \UnqCrashesHFPT & \UnqCrashesNNPT\\
    % \midrule\midrule
    % Diff. Tested &  - & \DiffTestedNNTF & \DiffTestedHFPT & \DiffTestedNNPT\\    
    % \midrule\midrule
    \bottomrule
    \end{tabular}
    \label{tab:RQ4ConversionConstrainedResults}
\end{table}
\fi

\subsection{RQ4: Converter Test Suites} \label{sec:res:RQ4}
\begin{tcolorbox} [width=\linewidth, colback=yellow!30!white, top=1pt, bottom=1pt, left=2pt, right=2pt]
\textbf{Finding 10}: 
The \code{tf2onnx} and \code{torch.onnx} converters employ both unit and end-to-end testing.
Unit testing focuses on individual operations.
End-to-end testing targets real models and utilizes differential testing to compare the original and converted models.

\textbf{Finding 11}: Test suites share few operators with mismatching models. Only 12 (20\%) with mismatching models for \code{torch.onnx}, while for \code{tf2onnx}, 33 (61\%) of operators are shared. Operators sequences are similar with only 2 (\code{torch.onnx}) and 35 (\code{tf2onnx}) sequences being shared with mismatching models.
\end{tcolorbox}

The \code{tf2onnx} and \code{torch.onnx} converters are both well-tested and have a variety of test suites written for them. 
As described in~\cref{sec:meth:testSuites} we examine the continuous integration and deployment pipelines and test files of each converter.
Both converters employ unit and end-to-end testing.
The unit testing targets the conversion of individual operations and functions, which can be thought of as sequences of operators.
These unit tests follow a structure similar to that presented in \cref{fig:MethodForRQ3DifferentialTest}.
A simple model is built with a single layer that is the operator or function being tested.
These models are then given a randomly generated input, and their output is stored.
The models are converted to ONNX, and that same input is provided to the ONNX model. The test is considered successful if both the output of the original and ONNX models are the same.
\code{tf2onnx} tests 41 operations and \code{torch.onnx} tests 164 operations and 470 functions.

The end-to-end testing targets fully developed models that will be commonly used by the ONNX converter.
Both frameworks pull various models from Hugging Face or libraries such as \code{Keras} and \code{torchvision.models} and attempt to convert them to ONNX.
\code{tf2onnx} tests a total of 88 real models and \code{torch.onnx} tests a total of 42 real models.
There are two suites of end-to-end tests for \code{tf2onnx}, the first, the older suite is more comprehensive than the second (96 as compared to 36).


The test suite models differ from the mismatching models.
Per~\cref{tab:RQ4AnalysisResultsNodes}, test suite models contain 16 (\code{torch.onnx}) and 54 (\code{tf2onnx}) unique operator types, but only 12  (\code{torch.onnx}) and 33 (\code{tf2onnx}) operators are shared with mismatched models.
Per~\cref{tab:RQ4AnalysisResultsSeq}, test suite models share only 2 (\code{torch.onnx}) and 35 (\code{tf2onnx}) sequences with mismatching models.
See implications in~\cref{sec:dis:conv_test}.

\section{Survey refugees}

\subsubsection{Preliminary Analysis}
\label{sec:theme0-prelimAnalysis}

%DL Intermediate Formats:
% \paragraph{DL Intermediate Formats}
% \textbf{DL Intermediate Formats:}
% Intermediate formats are a common intermediary to interoperate DL software.
We conducted a preliminary analysis on GitHub popularity statistics of interoperability tools.
\cref{tab:intermediate_formats} presents the common DL intermediate formats, including Open Neural Network eXchange (ONNX)~\citep{ONNXFixed}, NNEF~\citep{NNEF}, and MMdnn~\citep{MMdnn}.
ONNX has the broadest adoption with the most stars, forks, dependents, and packages utilizing it. %, with 
%ONNX boasts the most stars, forks, dependants, and packages utilizing it.

\section{Old Discussion}
\subsection{Simplifying DL Model Converter Engineering}

%{\centering
\begin{tcolorbox} [width=1.0\linewidth, colback=blue!07!white, top=1pt, bottom=1pt, left=2pt, right=2pt]

\textbf{OQ4}:
Is a small stable operator set a viable alternative?
%Can intermediaries such as ONNX be reduced to a limited set of operations and still represent all DL models?
%
\end{tcolorbox}
\vspace{-0.10cm}
%}

% It can be argued axiomatically that changes in common intermediaries can cause adapters to break.  
% Unsurprisingly this phenomenon is seen in ONNX converters, but not very strongly --- at least in a proportional or monotonic fashion.
% As presented in \cref{sec:res:RQ3} the relationship between ONNX operator set updates and converter failures is weakly monotonic.
% The reasons for this may be two-fold: converter designs are anti-fragile; failures greatly lag updates; or both.

% Converter designs may be anti-fragile by a combination of, operator changes being unequal in effect, and design and development practices. 
% The first follows from the fact that deep learning models are constructed from some fundamental operations, \eg matrix multiplication, addition, subtraction, and transposition. 
% These operators would be commonly by engineers and thus any converter that supports these ``fundamental operators" would to a degree work for ``common" inputs.
% Thus so long as newly added operations are not among the ``common" input the likelihood a failure would be reported would be low.
% The fact that converters support many operator sets would reduce failures caused by operator definitions being updated (\eg a new argument is supported).
% Such a decision would allow engineers to choose older operator sets that would not be ``breaking".

% Design and development practices are ONNX converters support conversion with older operator sets, so even if a change was breaking an engineer can choose not to use the latest operator set in the conversion.

% It may also be the case that the time delay between a new release and failures (as a result of that release) is large enough that a stronger relationship is not easily discernible. 
% This effect is convolved with "low-frequency operators", because if the effect of operator addition or update is unequal this would

\ifJOURNALEXTENSION
\JD{Discuss feedback loops: framework-ONNX, framework-converter, converter-ONNX. Tools to support.}
\fi


% In the current design of the ONNX specification, the ONNX operator set evolves to keep pace with changes in DL frameworks (\cref{fig:OpsetOverTime}, \eg~\citep{pytorchissue32960}).
% We found these changes to be correlated, weakly, with converter errors (\cref{sec:res:RQ3}).
% Error rates may be reduced by novel data and tools.
% For examples:
  % (1) Understanding operator popularity could focus validation efforts;
  % and
  % (2) A domain-specific language could generate converter code automatically.


Deep learning frameworks and accelerators continue to evolve, requiring interoperability software such as ONNX to continue to adapt.
New kinds of operators mean new failures --- our data show that node conversion errors are a common cause of failure (\cref{tab:causes}).
%operator set continues to evolve and so must converters to accommodate new operators (\cref{tab:causes}). 
The ONNX team is exploring one way to mitigate this class of error through \code{ONNXScript}~\citep{ONNXScript_Chu_2023}, a domain-specific language from which conversion code can be automatically generated.
Alternatively, we suggest exploring a small stable operator set. 
This approach differs from ONNX's in that it would express all higher-order operators as the composition of primitive ones.
A similar approach has been applied in other interoperability contexts, \eg the JVM bytecode~\citep{lindholm2014java} and the RISC architecture~\citep{patterson2016computer}.
% We find a weak positive correlation between the number of changes to the ONNX standard and the number of failures measured following the change.
% (\cref{sec:res:RQ3}).
%This indicates that converters are to a degree fragile to changes in ONNX and changes may result in subsequent converter updates to keep in line with ONNX.
%We also find evidence for this in our failure analysis~\citep{pytorchissue32960}, in that there exist feedback loops between frameworks, converters, and ONNX. 
%The addition of operations to a framework induces the need for converter support, and converter support induces the need for ONNX support.
%It is unknown how to mitigate the effects of this coupling but we believe tooling to extend converters may assist in reducing such effects.
%It is also unknown whether the design of ONNX is the right solution for DL interoperability, or would the ecosystem be better served through the creation of ``Reduced Operator Set" (ROS) (similar to RISC or JVM).
This design would introduce a (perhaps formally measurable) conversion error penalty in terms of latency (from non-customized operators) and accuracy (from approximation).
%It trades off translation complexity for a stable intermediate representation that reduces coupling.
%But such a design would reduce the effects of coupling and make converters robust to change.
% This suggests to us that future research should focus on techniques to extend converters to allow easy updates.
% Additionally, it is unknown whether changes are equal in effect, \ie if specific types of changes are more likely to cause failures, or whether there is a minimal intermediary that could support all DL models. 


% If this were the case, this would motivate study into a so-called ``Reduced Operator Set''. 
% \JD{...``similar to the RISC-V proposal''?}
% Such a construct could represent all DL models with a set of non-growing primitive operations, which as we show with \cref{fig:OpsetOverTime}, is not the case with ONNX.


% \textbf{Reduced Operator Set (ROS)}: \TODO{REVISE THIS} ONNX in its growth has seen an expansion of the number of operators supported. 
%     This expansion has consequently led to the extension of model converters to support these operators.
%     Though it is unknown how many of these operators are truly needed for interoperability. 
%     An open question remains whether or not a reduced operator set can be created that covers all possible operations in DL models. 
%     A reduced operator set, if possible, must be able to represent operations as one or more operations in the ROS.
%     Additionally, upon conversion to and from, it must maintain the semantics of the original model. 
%     The existence of a ROS would mean that converters would not have to update their mapping in accordance with new standards. Though it would increase the complexity of converters as a single node in the source graph would be equal to multiple nodes in the ROS graph, additionally, conversion from the ROS graph to a target representation would require knowledge of the boundaries (nodes) of the originally converted operator.

\ifARXIV
\else
%\vspace{-0.08cm}
\fi
% \subsection{From Bug Studies to Risk Analyses?}

% \begin{tcolorbox} [width=\linewidth, colback=blue!07!white, top=1pt, bottom=1pt, left=2pt, right=2pt]
% \textbf{OQ5}: Should the research community redefine the ``bug study''?
% \end{tcolorbox}
% %\vspace{-0.03cm}

% The purpose of software failure analysis research (``bug study'') is to understand the ways in which a given class of software fails~\citep{amusuo2022SoftwareFailureAnalysis}.
% The resulting knowledge informs engineers making decisions about designs or dependencies, and helps researchers identify trouble areas for further study.
% %The software engineering literature includes many ``bug studies'', examining defects that have already occurred.
% % but we agree with Amusuo \etal that we contend that 
% %Prior work focuses on taxonomizing defects, which sheds light on defect criticality.
% Prior work assesses failure criticality through taxonomies and impact analysis.
% However, it tends not to assess the likelihood of a failure. %nor identify causal factors beyond the ``root cause'' in the code.
% %We contend that while these studies are valuable, they do not actually provide software engineers or researchers with actionable information.
% %Engineers must make decisions.
% %Traditionally, failure analyses study failures retrospectively, \ie failures that have already happened~\citep{Amusuo_Sharma_Rao_Vincent_Davis_2022}. \WJ{When reading this sentence, I would like to know if our results have found new failures? If not, I don't think ``failures that have already happened'' is a good description here. I think it's better to use ``criticality'' (\$6.1) vs. ``Likelihood''.}
% %We suggest that the discipline should mature from bug studies to risk analyses.
% We innovate by combining a bug study (Theme 1) with an estimate of current failure presence (Theme 2), so that we may characterize the \emph{risks} of DL model converters (\cref{sec:dis:risks}).
% We wonder whether this risk-based approach to failure analysis yields more actionable information for engineers and researchers.
% %This is a divergence from what has been the tradition in failure analysis, in that, we not only characterize failure criticality but also likelihood. 
% %Traditionally, failure analyses study failures retrospectively, \ie failures that have already happened~\citep{Amusuo_Sharma_Rao_Vincent_Davis_2022}. \WJ{When reading this sentence, I would like to know if our results have found new failures? If not, I don't think ``failures that have already happened'' is a good description here. I think it's better to use ``criticality'' (\$6.1) vs. ``Likelihood''.}
% %This, as a picture of risks, is incomplete, in that to properly contextualize the risks to a system we must measure how often it fails. 
% %In fact, traditional failure analyses cannot characterize the risks associated with a piece of software because they lack information on the \emph{likelihood} of failures.

\ifARXIV
\else
%\vspace{-0.1cm}
\fi

\vspace{-5pt}

\begin{table}
\caption{
  Popularity of DL intermediate formats.
  ONNX has the most stars, forks, dependents, and Stack Overflow posts.
  Data from August 12, 2023.
}
\small
\begin{tabular}{crrrr}
\toprule
\textbf{Project} 
& \textbf{Stars}  
& \textbf{Forks}  
& \textbf{Deps.}
%& \textbf{Pkgs.}
& \textbf{Posts}
\\ \hline
\code{ONNX}~\citep{ONNXFixed}     
& 14,859   
& 3,534 
& 15,728 
%& 479
& 1148       \\
\code{MMdnn}~\citep{MMdnn}        
& 5,726    
& 980 
& 110   
%& 0
& 24          \\
\code{NNEF}~\citep{NNEF}       
& 206    
& 51  
& 0
%& 0           
& 1           \\
\bottomrule
\end{tabular}
\label{tab:intermediate_formats}
% \end{wraptable}
\end{table}

\section{The joint distribution table, not done tiny}
\begin{table*}
    %\small
    \caption{
    Joint distribution of causes and symptoms.
    We bold notable occurrences and drop the \emph{Concurrency} and \emph{Documentation} rows because they contain all zeros. 
    The majority of \emph{Crashes} result from \emph{Incompatibilities} and \emph{Type Problems}.
    \emph{Algorithmic Errors} that result in \emph{Wrong Models} occur more often in \code{tf2onnx}.
    The top-5 causes in terms of frequency are shown, with the rest binned as \emph{Others} category. The \emph{Others} are \emph{Concurrency}, \emph{Docs}, \emph{Incorrect Numerical Computation}, \emph{Misconfig}, \emph{Testing}, \emph{Incorrect Exception Handling}, \emph{Typos}, and \emph{Incorrect Assignment}.
    }
    % Space
    %\small
% \begin{tabular}{l|cc|cc|cc|cc|cc||cc}
% \toprule
% \multirow{2}{*}{\backslashbox[15em]{Causes}{Symptoms}} & \multicolumn{2}{c|}{Crash} & \multicolumn{2}{c|}{Wrong Model} & \multicolumn{2}{c|}{Bad Performance} & \multicolumn{2}{c|}{Build Failure} & \multicolumn{2}{c||}{Unreported} & \multicolumn{2}{c}{Total} \\
% {} &    PT &  TF &         PT &  TF &              PT & TF &            PT & TF &         PT &  TF &    PT &   TF \\
% \midrule
% API Misuse                      &     5 &   6 &          1 &   0 &               0 &  0 &             0 &  0 &          0 &   0 &     \emph{6} &    \emph{6} \\
% Incompatibility                 &    \textbf{28} &  \textbf{19} &          3 &   4 &               0 &  0 &             0 &  0 &          1 &   2 &    \emph{32} &   \emph{25} \\
% Type Problem                    &    \textbf{14} &   \textbf{8} &         \textbf{13} &  \textbf{17} &               1 &  0 &             0 &  0 &          1 &   0 &    \emph{29} &   \emph{25} \\
% Shape Problem                   &     4 &   5 &          7 &   4 &               0 &  0 &             0 &  0 &          1 &   0 &    \emph{12} &    \emph{9} \\
% Incorrect Numerical Computation &     0 &   0 &          0 &   0 &               0 &  0 &             0 &  0 &          0 &   0 &     \emph{0} &    \emph{0} \\
% Incorrect Assignment            &     2 &   0 &          0 &   0 &               0 &  0 &             0 &  0 &          0 &   0 &     \emph{2} &    \emph{0} \\
% Incorrect Exception Handling    &     1 &   1 &          1 &   0 &               0 &  0 &             0 &  0 &          0 &   0 &     \emph{2} &    \emph{1} \\
% Misconfiguration                &     0 &   1 &          0 &   0 &               0 &  0 &             2 &  2 &          0 &   1 &     \emph{2} &    \emph{4} \\
% % Concurrency                     &     0 &   0 &          0 &   0 &               0 &  0 &             0 &  0 &          0 &   0 &     0 &    0 \\
% Algorithmic Error               &     3 &   4 &          \textbf{3} &  \textbf{10} &               0 &  2 &             0 &  0 &          0 &   2 &     \emph{6} &   \emph{18} \\
% Typo                            &     2 &   0 &          0 &   0 &               0 &  0 &             0 &  1 &          0 &   0 &     \emph{2} &    \emph{1} \\
% Testing                         &     1 &   0 &          1 &   0 &               0 &  0 &             0 &  0 &          1 &   1 &     \emph{3} &    \emph{1} \\
% % Documentation                   &     0 &   0 &          0 &   0 &               0 &  0 &             0 &  0 &          0 &   0 &     0 &    0 \\
% Others                          &     2 &   6 &          1 &   0 &               0 &  0 &             0 &  0 &          1 &   4 &     \emph{4} &   \emph{10} \\
% \midrule\midrule
% \emph{Total}                    &    \emph{62} &  \emph{50} &         \emph{30} &  \emph{35} &        \emph{1} &  \emph{2} &    \emph{2} &  \emph{3} &          \emph{5} &  \emph{10} &   \emph{100} &  \emph{100} \\
% \bottomrule
% \end{tabular}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{l|rr|rr|rr|rr|rr||rr}
\toprule
%\multirow{2}{*}{\backslashbox[15em]{Causes}{Symptoms}} & \multicolumn{2}{c|}{Crash} & \multicolumn{2}{c|}{Wrong Model} & \multicolumn{2}{c|}{Bad Performance} & \multicolumn{2}{c|}{Build Failure} & \multicolumn{2}{c||}{Unreported} & \multicolumn{2}{c}{Total} \\
\multirow{2}{*}{\textbf{Cause}} & \multicolumn{2}{c|}{\textit{Crash}} & \multicolumn{2}{c|}{\textit{Wrong Model}} & \multicolumn{2}{c|}{\textit{Bad Performance}} & \multicolumn{2}{c|}{\textit{Build Failure}} & \multicolumn{2}{c||}{\textit{Unreported}} & \multicolumn{2}{c}{\textit{Total}} \\
{} &    TF &  PT &         TF &  PT &              TF & PT &            TF & PT &         TF & PT &    TF &   PT \\
\midrule
Incompatibility                 &    \textbf{19} &  \textbf{28} &          4 &   3 &               0 &  0 &             0 &  0 &          2 &  1 &    \emph{25} &   \emph{32} \\
Type Problem                    &     \textbf{8} &  \textbf{14} &         \textbf{17} &  \textbf{13} &               0 &  1 &             0 &  0 &          0 &  1 &    \emph{25} &   \emph{29} \\
Algorithmic Error               &     4 &   3 &         \textbf{10} &   \textbf{3} &               2 &  0 &             0 &  0 &          2 &  0 &    \emph{18} &    \emph{6} \\
Shape Problem                   &     5 &   4 &          4 &   7 &               0 &  0 &             0 &  0 &          0 &  1 &     \emph{9} &   \emph{12} \\
API Misuse                      &     6 &   5 &          0 &   1 &               0 &  0 &             0 &  0 &          0 &  0 &     \emph{6} &    \emph{6} \\
Others                          &    \BinnedJointOtherCrashTF &   \BinnedJointOtherCrashPT &          \BinnedJointOtherWrongModelTF &   \BinnedJointOtherWrongModelPT &               \BinnedJointOtherBadPerfTF &  \BinnedJointOtherBadPerfPT &  \BinnedJointOtherBuildFailTF &  \BinnedJointOtherBuildFailPT &    \BinnedJointOtherUnreportedTF & \BinnedJointOtherUnreportedPT  &  \emph{\BinnedOtherTF} &    \emph{\BinnedOtherPT} \\
% Misconfiguration                &     1 &   0 &          0 &   0 &               0 &  0 &             2 &  2 &          1 &  0 &     4 &    2 \\
% Incorrect Exception Handling    &     1 &   1 &          0 &   1 &               0 &  0 &             0 &  0 &          0 &  0 &     1 &    2 \\
% Typo                            &     0 &   2 &          0 &   0 &               0 &  0 &             1 &  0 &          0 &  0 &     1 &    2 \\
% Testing                         &     0 &   1 &          0 &   1 &               0 &  0 &             0 &  0 &          1 &  1 &     1 &    3 \\
% Incorrect Numerical Computation &     0 &   0 &          0 &   0 &               0 &  0 &             0 &  0 &          0 &  0 &     0 &    0 \\
% Incorrect Assignment            &     0 &   2 &          0 &   0 &               0 &  0 &             0 &  0 &          0 &  0 &     0 &    2 \\
% Concurrency                     &     0 &   0 &          0 &   0 &               0 &  0 &             0 &  0 &          0 &  0 &     0 &    0 \\
% Documentation                   &     0 &   0 &          0 &   0 &               0 &  0 &             0 &  0 &          0 &  0 &     0 &    0 \\
\midrule\midrule
Total                           &    \emph{50} &  \emph{62} &         \emph{35} &  \emph{30} &               \emph{2} &  \emph{1} &             \emph{3} &  \emph{2} &         \emph{10} &  \emph{5} &   \emph{100} &  \emph{100} \\
\bottomrule
\end{tabular}
%}
\label{tab:cau_sym}
\end{table*}

\clearpage

\section{Move this to supplement but not in the paper itself}
{
\small
\begin{table}[]
    \footnotesize
    \caption{\small
        Distribution of causes in \code{tf2onnx} and \code{torch.onnx}.
        The top-5 causes in terms of frequency are shown. 
        The \emph{Others} are: \emph{Concurrency}, \emph{Documentation}, \emph{Incorrect Numerical Computation}, \emph{Misconfiguration}, \emph{Testing}, \emph{Incorrect Exception Handling}, \emph{Typos}, and \emph{Incorrect Assignment} (each has $<3$\% representation).
        The final column shows the cause distribution from Shen \etal~\citep{DLcompilerbugs}.
        Note the larger proportion of \emph{Incompatibility} failures in DL model converters (first row).
        \JD{This table is formatted real weird}
        \NJE{I think it would look fine without vertical bars. Sadly LaTeX doesn't like multirow + the "c" option.}
        \GKT{Oddly, I like the table but worry that most readers are going to get lost with our sentence "notable aspects". Let's be clear about what this table is telling the reader and not make them search for "the text" and no x-ref.}
        \WJ{This table has ``incompatibility resource'' but it's not in table 7. Make sure it's consistent.}
        }
    % Space
    % \small
    \begin{tabular}{l|c|r|r||r||p{1.6cm}}
    \toprule
    \multicolumn{2}{c|}{\textbf{Causes}}                          &  \textbf{TF} &  \textbf{PT} &  \textbf{Total} & \textbf{Comp. to DL compilers}~\citep{DLcompilerbugs}\\
    \toprule
    \multirow{3}{*}{Incompatibility}    
                                         &      External &       \textbf{23} &       \textbf{32} &     \textbf{55 (\IncompExt)} &  \ShenIncompExt (\ShenIncompExtPercent)\\  
    &      Internal &        2 &        0 &      2 (\IncompInt) & \ShenIncompInt (\ShenIncompIntPercent) \\
                                         &      Resource &        0 &        0 &      0 (\IncompRes) & \ShenIncompRes (\ShenIncompResPercent)\\  
    \midrule
    \multirow{3}{*}{Type Problem}        &          Node &       \textbf{21} &       \textbf{25} &     \textbf{46 (\TypeNode)} & \ShenTypeNode (\ShenTypeNodePercent)\\
                                         &  Conventional &        3 &        2 &      5 (\TypeConv) & \ShenTypeConv (\ShenTypeConvPercent)\\
                                         &        Tensor &        1 &        2 &      3 (\TypeTensor) & \ShenTypeTens(\ShenTypeTensPercent)\\  
    \midrule
    \multicolumn{2}{c|}{Algorithmic Error}               &       \textbf{18} &        \textbf{6} &     \textbf{24 (\Algo)} & \ShenAlgo (\ShenAlgoPercent) \\
    \midrule
    \multicolumn{2}{c|}{Shape Problem}                   &       9 &        12 &     21 (\Shape) & \ShenShape (\ShenShapePercent) \\
    \midrule
    \multicolumn{2}{c|}{API Misuse}                        &        6 &        6 &     12 (\API) & \ShenAPI (\ShenAPIPercent) \\
    % \midrule
    % \multicolumn{2}{c|}{Misconf.}                        &        4 &        2 &      6 (\Misconf)\\
    % \midrule
    % \multicolumn{2}{c|}{Testing}                         &        1 &        3 &      4 (\Testing)\\
    % \midrule
    % \multicolumn{2}{c|}{Inc. Except. Handling}           &        1 &        2 &      3 (\IncExceptHandling)\\
    % \midrule
    % \multicolumn{2}{c|}{Typo}                            &        1 &        2 &      3 (\Typo)\\
    % \midrule
    % \multicolumn{2}{c|}{Inc. Assign.}                    &        0 &        2 &      2 (\IncAssign) \\
    % \midrule
    % \multicolumn{2}{c|}{Inc. Num. Comp.}                 &        0 &        0 &      0 (0\%)\\
    % \midrule
    % \multicolumn{2}{c|}{Concurrency}                     &        0 &        0 &      0 (0\%)\\
    % \midrule
    % \multicolumn{2}{c|}{Documentation}                   &        0 &        0 &      0 (0\%)\\
    \midrule
    \multicolumn{2}{c|}{Others}                          &       \BinnedOtherTF & \BinnedOtherPT &     \BinnedOther (\BinnedOtherPercentage) & \ShenOthers(\ShenOthersPercent) \\
    % \midrule 
    \midrule
    \midrule
    \multicolumn{2}{c|}{\emph{Total}}                           &      \emph{100} &      \emph{100} &    \emph{200 (100\%)} &  \emph{\ShenTotalCauses (\ShenTotalCausesPercent)}\\  
    \bottomrule
    \end{tabular}
    \label{tab:causes}
\end{table}
}

\section{Refugee table from 6.2.4 --- not interesting enough to include}

\begin{table}[ht!]
    \centering
% \begin{wraptable}{r}{0.45\columnwidth}
    \caption{\small
    Model Operator Analysis Results.
    As described in~\cref{sec:meth:H3}: 
    Mismatched $\circledstep{1}$, all operators that mismatched models contain; 
    Correct $\circledstep{2}$ all operators that correct models contain;
    Test Suite $\circledstep{3}$ all operators that test suites contain.
    $\circledstep{1} \setminus \circledstep{2}$ are all operators in $\circledstep{1}$ but not in $\circledstep{2}$.
    $\circledstep{2} \setminus \circledstep{1}$ are all operators in $\circledstep{2}$ but not in $\circledstep{1}$.
    $\circledstep{1} \setminus \circledstep{3}$ are all operators in $\circledstep{1}$ but not in $\circledstep{3}$.
    $\circledstep{3} \setminus \circledstep{1}$ are all operators in $\circledstep{3}$ but not in $\circledstep{1}$.
    % \circledstep{4} - \circledstep{2} are all unique sequences that are \emph{only} present in test suite models.
    % The reduced sequences are found by applying the reduction as described in~\cref{sec:meth:model_analysis}
    }
   % Reduce font size?
   \small
    \begin{tabular}{c|r|r}
    \toprule
    \textbf{Model Type}   &  \emph{\textbf{\code{tf2onnx}}} &  \emph{\textbf{\code{torch.onnx}}} \\
    \midrule
    Mismatched $\circledstep{1}$ &   54  & 58 \\
    Correct $\circledstep{2}$ &    52  & 59 \\
    Test Suite $\circledstep{3}$ &   54 & 16\\
    \midrule
    $\circledstep{1} \setminus \circledstep{2}$ &   0  & 1 \\
    $\circledstep{2} \setminus \circledstep{1}$ &   2  & 0 \\
    $\circledstep{1} \setminus \circledstep{3}$ &   21  & 46 \\
    $\circledstep{3} \setminus \circledstep{1}$ &   21  & 4 \\
    \bottomrule
    \end{tabular}
    \label{tab:RQ4AnalysisResultsNodes}
%\vspace{-0.15cm}
\end{table}

\subsection{StackOverflow}

% Survey Data.
\begin{table}
\caption{
  \PJ{REPLACE WITH WENXIN SURVEY DATA} Goals of ONNX posts on StackOverflow. %belonging to the category Conceptual, Development, Deployment, Unclear, or N/A.
  }
\small
  \vspace{-0.25cm}
\begin{tabular}{cr}
\toprule
\textbf{Goal} 
& \textbf{\# Posts}  
\\ \hline
Conceptual  
& 1  
\\
Development
& 1  
\\
Deployment       
& 36
\\
Unclear
& 27
\\
N/A
& 2
\\
\midrule
\textbf{Total} 
& 67
\\
\bottomrule
\end{tabular}
\label{tab:stackoverflow}
\end{table}
